Infrared Spectroscopy of free-floating planet candidates in Upper Scorpius and Ophiuchus

Context: A rich population of low-mass brown dwarfs and isolated planetary mass objects has been reported recently in the Upper Scorpius and Ophiuchus star forming complex. Aims: We investigate the membership, nature and properties of 17 of these isolated planetary mass candidates using low-resolution near-infrared spectra. Methods: We investigate the membership by looking for evidences of youth using four diagnostics: the slope of the continuum between the J and Ks band, the Hcont and TLI-g gravity sensitive indices, and by comparing the spectra to young and field (old) M and L-dwarf standards. Results: All the targets but one are confirmed as young ultracool objects, with spectral types between L0 and L6 and masses in the range 0.004-0.013 M according to evolutionary models. The status of the last target is unclear at this point. Conclusions: Only one possible contaminant has been identified among the 17 targets, suggesting that the contamination level of the original sample must be lower than 6%

==> Upper Sco Spectra/Tables/all_indices.tex <==
\begin{table}
\centering
\caption{Gravity sensitive indices measured in 891 spectra of the SPEX library \label{tab_all_indices}}
\begin{tabular}{lcccccccc}
\hline
Name & RA (J2000) & Dec (J2000) & SpT & \texttt{SPEX\_CLASS} & H$_{\rm cont}$ &  e\_H$_{\rm cont}$ & TLI-g & e\_TLI-g \\
\hline
    2MASS J0000286-124515 & 0.11945834 & -12.75425 & M9.0 & FLD-G & 0.947 & 0.003 & 1.015 & 0.01\\
  2MASS J00013044+1010146 & 0.37683335 & 10.170723 & M6.0 & VL-G & 0.988 & 0.006 & 1.009 & 0.023\\
  LHS 102B & 1.1451666 & -40.734943 & L4.0 & FLD-G & 0.855 & 0.002 & 1.011 & 0.008\\
  LEHPM 1-162 & 1.4486667 & -21.954889 & M8.0 & FLD-G & 0.963 & 0.002 & 0.994 & 0.009\\
  2MASSI J0006205-172051 & 1.5854167 & -17.347389 & L2.0 & FLD-G & 0.897 & 0.006 & 0.998 & 0.006\\
  SDSS J000632.60+140606.4 & 1.6358334 & 14.101778 & L1.0 & FLD-G & 0.931 & 0.009 & 0.989 & 0.017\\
  SDSS J000649.16-085246.3 & 1.7048334 & -8.879528 & M8.0 & FLD-G & 0.921 & 0.004 & 1.035 & 0.008\\
  2MASS J0007078-245804 & 1.7827917 & -24.967834 & M8.0 & INT-G & 0.987 & 0.003 & 1.008 & 0.017\\
  2MASS J00085931+2911521 & 2.2471251 & 29.197805 & M8.0 & INT-G & 0.967 & 0.002 & 1.013 & 0.007\\
  2MASS J00100009-2031122 & 2.500375 & -20.520056 & M8.0 & FLD-G & 0.933 & 0.003 & 1.049 & 0.003\\
  2MASSI J0013578-223520 & 3.4907918 & -22.58889 & L5.0 & FLD-G & 0.859 & 0.01 & 0.992 & 0.01\\
  WISE J001450.14-083823.1 & 3.7089167 & -8.6397219 & M7.0 & FLD-G & 0.945 & 0.008 & 1.042 & 0.016\\
  2MASS J00145575-4844171 & 3.7322917 & -48.738083 & L3.0 & FLD-G & 0.883 & 0.006 & 1.022 & 0.013\\
  2MASSW J0015447+351603 & 3.9364998 & 35.267387 & L2.0 & INT-G & 0.9 & 0.003 & 1.025 & 0.006\\
  SDSS J001608.44-004302.3 & 4.0351253 & -0.71722221 & L3.0 & INT-G & 0.898 & 0.008 & 0.961 & 0.023\\
  2MASS J00163761+3448368 & 4.1567087 & 34.810223 & M8.0 & FLD-G & 0.939 & 0.004 & 1.016 & 0.013\\
\hline\end{tabular}
\end{table}

==> Upper Sco Spectra/Tables/indices.tex <==
\begin{table}
\centering
\caption{Gravity sensitive indices \label{tab_indices}}
\begin{tabular}{ccc}
\hline
Object & H$_{\rm cont}$ & TLI-g \\
\hline
  3091 & 0.97$\pm$0.05 & 0.84$\pm$0.05\\
  3144 & 0.99$\pm$0.07 & 1.03$\pm$0.07\\
  3200 & 1.01$\pm$0.03 & 0.95$\pm$0.04\\
  3210 & 0.99$\pm$0.03 & 0.97$\pm$0.03\\
  3213 & 0.92$\pm$0.05 & 0.85$\pm$0.05\\
  3214 & 0.96$\pm$0.09 & 0.97$\pm$0.07\\
  3231 & 0.93$\pm$0.03 & 0.92$\pm$0.03\\
  3244 & 0.94$\pm$0.03 & 0.90$\pm$0.02\\
  3293 & 0.93$\pm$0.03 & 0.95$\pm$0.03\\
  3299 & 0.94$\pm$0.03 & 0.91$\pm$0.03\\
  3314 & 0.99$\pm$0.02 & 0.93$\pm$0.02\\
  3324 & 0.96$\pm$0.02 & 0.98$\pm$0.02\\
  3326 & 0.99$\pm$0.04 & 0.92$\pm$0.04\\
  3345 & 0.99$\pm$0.05 & 0.86$\pm$0.05\\
  3355 & 0.96$\pm$0.04 & 0.90$\pm$0.05\\
  3378 & 0.91$\pm$0.12 & 0.93$\pm$0.14\\
  3404 & 0.84$\pm$0.10 & 0.96$\pm$0.15\\
  3421 & 0.93$\pm$0.03 & 0.94$\pm$0.03\\
\hline\end{tabular}
\end{table}

==> Upper Sco Spectra/Tables/old_std.tex <==
\begin{table*}
\caption{Library of field ultracool standards \label{old_stds}}
\begin{tabular}{lcccc}
\hline
  Name &  RA (J2000) &  Dec (J2000) &  SpT &  Ref. \\
\hline
  VB 10 & 289.2400917 & 5.1506056 & M8 & (2)\\
  LP 944-20 & 54.89675 & -35.4289139 & L0 & (1) \\
  GJ 1048B & 38.9997083 & -23.5223611 & L1 & (1)\\
  2MASSI J2057540-025230 & 314.4753917 & -2.8750722 & L2 & (2)\\
  2MASSW J1506544+132106 & 226.7267125 & 13.3516889 & L3 & (3)\\
  2MASSW J0036159+182110 & 9.0674 & 18.3529083 & L4 & (1) \\
  SDSSp J144600.60+002452.0 & 221.5025833 & 0.4144444 & L5 & (4) \\
  2MASSI J1010148-040649 & 152.5616958 & -4.1138694 & L6 & (5) \\
  2MASSI J1526140+204341 & 231.5585417 & 20.7281833 & L7 & (2)\\
\hline\end{tabular}
\tablebib{(1) \citet{Burgasser2008} ; (2) \citet{Burgasser2004} ; (3) \citet{Burgasser2007} ; (4) \citet{Bardalez2014} ; (5) \citet{Reid2006} }
\end{table*}

==> Upper Sco Spectra/Tables/splat_vlg_std.tex <==
\begin{table*}
\caption{SPEX library of very-low gravity ultracool standards \label{splat_stds}}
\begin{tabular}{lcccc}
\hline
  Name & RA & Dec & SpT & Ref. \\
\hline
  2MASSW J1207334-393254A & 181.88959 & -39.548443 & M8 & (1) \\
  TWA 26 & 174.96304 & -31.989279 & M9 & (1) \\
  2MASS J01415823-4633574 & 25.492626 & -46.565945 & L0$\gamma$ & (2)\\
  2MASS J05184616-2756457 & 79.692337 & -27.946028 & L1$\gamma$ & (3)\\
  2MASS J05361998-1920396 & 84.083244 & -19.344334 & L2$\gamma$ & (3)\\
  2MASSW J2208136+292121 & 332.05679 & 29.355972 & L3$\gamma$ & (2)\\
  2MASS J05012406-0010452 & 75.35025 & -0.17922223 & L4$\gamma$ & (2)\\
  2MASSW J2244316+204343 & 341.13196 & 20.728695 & L7$\gamma$ & (4) \\
\hline\end{tabular}
\tablebib{(1) \citet{Gizis2002} ; (2) \citet{Cruz2009} ; (3) \citet{Bardalez2014} ; (4) \citet{Kirkpatrick2008}}
\end{table*}


==> Upper Sco Spectra/Tables/spt.tex <==
\begin{table}
\centering
\caption{Adopted spectral types and estimated effective temperatures and masses for the confirmed members. \label{tab_spt}}
\scriptsize
\begin{tabular}{cccccc}
\hline
  ID &   SpT & T$_{\rm eff}$     & Mass 3Myr & Mass 6Myr & Mass 10Myr \\
     &       &  (K)              & (M$_{\odot}$) & (M$_{\odot}$) & (M$_{\odot}$)\\
\hline
3213 & L2 & 1880                          & 0.007     & 0.010 & 0.012 \\
3214 & L2--L4 & 1560--1880      & 0.005--0.007       & 0.007--0.010 & 0.009--0.012 \\
3345 & L6 & 1220                          & 0.003     & 0.004& 0.006 \\
3355 & L1--L3 & 1740--1970                & 0.006--0.008     & 0.008--0.011& 0.011--0.013 \\
3378 & L2--L4 & 1560--1880                & 0.005--0.007     & 0.007--0.010 & 0.009--0.012 \\
3404 & L3--L4 & 1560--1740                & 0.005--0.006     & 0.007--0.008 & 0.009--0.011 \\
3314 & L0 & 2060 		          & 0.009     & 0.012& 0.014 \\
3231 & L1 & 1970  		          & 0.008     & 0.011& 0.013 \\
3091 & L0 & 2060   	                  & 0.009     & 0.012& 0.014 \\
3210 & L0 & 2060  		          & 0.009     & 0.012& 0.014 \\
3244 & L1 & 1970 		          & 0.008     & 0.011& 0.013 \\
3421 & L1 & 1970 		          & 0.008     & 0.011& 0.013 \\
3326 & L2 & 1880  		          & 0.007     & 0.010 & 0.012 \\
3144 & L4 & 1560 		          & 0.005     & 0.007& 0.009 \\
3200 & L0 & 2060  		          & 0.009     & 0.012& 0.014 \\
3299 & L4 & 1560                          & 0.005     & 0.007& 0.009 \\
\hline
\end{tabular}
\end{table}

==> Upper Sco Spectra/Tables/targets.tex <==
\begin{table*}
\centering
\caption{Targets observed
\label{tab_targets}}
\scriptsize
\begin{tabular}{cccccccccccc}
\hline
  Name & ID\tablefootmark{a} &   RA &   Dec &   $A_v$ max. &   i   & z &  y &   J  &   H  &   Ks  & Exp. Time \\
     & & (J2000) & (J2000) & mag     & mag  & mag   & mag  & mag & mag  & mag   & \texttt{NDIT$\times$DIT} s \\
\hline
\multicolumn{12}{c}{SWIMS} \\
\hline
DANCe J16135217-2443562  &  3213 & 16:13:52.17 & -24:43:56.2 & 0.82 & 23.76$\pm$0.13 & 22.03$\pm$0.05 & 21.52$\pm$0.06 & 18.84$\pm$0.06 & 17.70$\pm$0.05 & 16.70$\pm$0.05 & 40$\times$300\\				   
DANCe J16134589-2442310  &  3214 & 16:13:45.89 & -24:42:31.0 & 0.82 & 23.72$\pm$0.20 & 22.05$\pm$0.06 & 21.37$\pm$0.05 & 19.17$\pm$0.08 & 17.73$\pm$0.05 & 16.81$\pm$0.05 & 36$\times$300\\				   
DANCe J16081299-2304316  &  3345 & 16:08:12.99 & -23:04:31.6 & 0.52 & 23.69$\pm$0.08 & 22.01$\pm$0.05 & 22.15$\pm$0.08 & 18.94$\pm$0.05 & 17.80$\pm$0.05 & 16.82$\pm$0.05 & 24$\times$300\\				   
DANCe J16064553-2121595  &  3355 & 16:06:45.53 & -21:21:59.5 & 0.49 & 21.03$\pm$0.05 & 19.11$\pm$0.05 & 18.40$\pm$0.05 & 16.19$\pm$0.05 & 15.31$\pm$0.05 & 14.55$\pm$0.05 & 8$\times$300\\				   
DANCe J16091010-1930376  &  3378 & 16:09:10.10 & -19:30:37.6 & 0.60 & 24.09$\pm$0.11 & 22.19$\pm$0.05 & 21.58$\pm$0.05 & 19.03$\pm$0.09 & 17.81$\pm$0.05 & 16.74$\pm$0.05 & 22$\times$300\\				   
DANCe J15454024-2422072  &  3404 & 15:45:40.24 & -24:22:07.2 & 0.74 & 23.41$\pm$0.10 & 21.99$\pm$0.07 &$\cdots$ & 18.55$\pm$0.06 & 17.55$\pm$0.05 & 16.67$\pm$0.05 & 22$\times$300\\		
\hline
\multicolumn{12}{c}{EMIR} \\
\hline  
DANCe J16221885-2440029  &  3293 & 16:22:18.85 & -24:40:02.9 & 2.99 & 22.20$\pm$0.05 & 20.42$\pm$0.05 & 19.70$\pm$0.05 & 17.33$\pm$0.05 & 16.25$\pm$0.05 & 15.48$\pm$0.05 & 16$\times$200\\				   
DANCe J16064467-2033428  &  3314 & 16:06:44.67 & -20:33:42.8 & 0.77 & 22.29$\pm$0.05 & 20.45$\pm$0.05 & 19.85$\pm$0.05 & 17.56$\pm$0.05 & 16.50$\pm$0.05 & 15.72$\pm$0.05 & 28$\times$200\\				   
DANCe J16140756-2211524  &  3231 & 16:14:07.56 & -22:11:52.4 & 0.63 & 23.02$\pm$0.05 & 21.09$\pm$0.05 & 20.78$\pm$0.05 & 18.28$\pm$0.05 & 17.28$\pm$0.05 & 16.44$\pm$0.05 & 24$\times$200\\				   
DANCe J16255679-2113354  &  3091 & 16:25:56.79 & -21:13:35.4 & 1.81 & 23.53$\pm$0.11 & 21.76$\pm$0.05 & 21.19$\pm$0.06 & 18.39$\pm$0.08 & 17.33$\pm$0.05 & 16.36$\pm$0.05 & 28$\times$200\\				   
DANCe J16123953-2614510  &  3210 & 16:12:39.53 & -26:14:51.0 & 0.88 & 23.05$\pm$0.14 &$\cdots$& 20.24$\pm$0.05 & 18.43$\pm$0.06 & 17.31$\pm$0.05 & 16.34$\pm$0.05 & 24$\times$200\\			   
DANCe J16053908-2403330  &  3244 & 16:05:39.08 & -24:03:33.0 & 0.36 & 23.14$\pm$0.07 & 21.40$\pm$0.05 & 20.87$\pm$0.07 & 18.47$\pm$0.05 & 17.33$\pm$0.05 & 16.33$\pm$0.05 & 32$\times$200\\				   
DANCe J16020000-2057342  &  3324 & 16:02:00.00 & -20:57:34.2 & 0.66 & 23.15$\pm$0.05 & 21.66$\pm$0.05 & 21.11$\pm$0.05 & 18.54$\pm$0.05 & 17.50$\pm$0.05 & 16.35$\pm$0.05 & 32$\times$200\\				   
DANCe J16393029-2454135  &  3421 & 16:39:30.29 & -24:54:13.5 & 0.69 & 23.36$\pm$0.07 & 21.69$\pm$0.06 & 20.82$\pm$0.05 & 18.55$\pm$0.05 & 17.44$\pm$0.05 & 16.59$\pm$0.05 & 32$\times$200\\				   
DANCe J16041234-2127472  &  3326 & 16:04:12.34 & -21:27:47.2 & 0.52 & 23.69$\pm$0.07 & 21.91$\pm$0.05 & 21.53$\pm$0.05 & 18.70$\pm$0.05 & 17.43$\pm$0.05 & 16.57$\pm$0.05 & 32$\times$200\\				   
DANCe J16254583-2347372  &  3144 & 16:25:45.83 & -23:47:37.2 & 3.21 & 23.64$\pm$0.14 & 21.93$\pm$0.06 & 21.42$\pm$0.05 & 18.74$\pm$0.05 & 17.49$\pm$0.05 & 16.46$\pm$0.05 & 46$\times$200\\				   
DANCe J15481655-2307430  &  3200 & 15:48:16.55 & -23:07:43.0 & 0.77 & 23.65$\pm$0.12 &$\cdots$&$\cdots$& 18.76$\pm$0.09 & 17.50$\pm$0.05 & 16.56$\pm$0.05 & 32$\times$200\\			   
DANCe J15582895-2530319  &  3299 & 15:58:28.95 & -25:30:31.9 & 0.36 & 23.70$\pm$0.12 & 22.01$\pm$0.05 & 21.41$\pm$0.06 & 18.76$\pm$0.06 & 17.40$\pm$0.05 & 16.41$\pm$0.05 & 32$\times$200\\                            
\hline
\end{tabular}
\tablefoot{$A_v$ max. corresponds to the integrated line-of-sight interstellar reddening to 250~pc in the direction of the source as computed by \citet{Green2019}. {\bf The near-infrared JHKs photometry comes in the 2MASS system.}\\
\tablefoottext{a}{From \citet{2022NatAs...6...89M}}}
\end{table*}

==> Upper Sco Spectra/Tables/youth.tex <==
\begin{table}
\centering

\caption{Diagnostics of youth  \label{tab_youth}}
\begin{tabular}{cccccc}

\hline
  ID &   $J-Ks$ & Comparison    &     H$_{\rm cont}$ & TLI-g & Young?   \\
     &          & with standard &                    &       &     \\
\hline
  3091 & Young & Young  & Young & Young & Young\\
  3144 & Young & Young  & Young & Old   & Young\\
  3200 & Young & Young  & Young & Young & Young\\
  3210 & Young & Young  & Young & Young & Young\\
  3213 & Young & Young  & ?     & Young & Young\\
  3214 & Young & Young  & Young & Young & Young\\
  3231 & Young & Young? & Int?  & Young & Young\\
  3244 & Young & Young? & Int?  & Young & Young\\
  3293 & Young & Old?   & Old?  & Young & ?    \\
  3299 & Young & Young  & Young & Young & Young\\
  3314 & Young & Young  & Young & Young & Young\\
  3326 & Young & Young  & Young & Young & Young\\
  3345 & Young & Young  & Young & Young & Young\\
  3355 & Young & Young  & Young & Young & Young\\
  3378 & Young & Young  & ?     & ?     & Young\\
  3404 & Young & Young? & Old?  & ?     & Young\\
  3421 & Young & Young? & Int?  & Young & Young\\
\hline
\end{tabular}
\end{table}
